Committee Selection with Attribute Level Preferences

We consider the problem of committee selection from a fixed set of candidates where each candidate has multiple quantifiable attributes. To select the best possible committee, instead of voting for a candidate, a voter is allowed to approve the preferred attributes of a given candidate. Though attribute based preference is addressed in several contexts, committee selection problem with attribute approval of voters has not been attempted earlier. A committee formed on attribute preferences is more likely to be a better representative of the qualities desired by the voters and is less likely to be susceptible to collusion or manipulation. In this work, we provide a formal study of the different aspects of this problem and define properties of weak unanimity, strong unanimity, simple justified representations and compound justified representation, that are required to be satisfied by the selected committee. We show that none of the existing vote/approval aggregation rules satisfy these new properties for attribute aggregation. We describe a greedy approach for attribute aggregation that satisfies the first three properties, but not the fourth, i.e., compound justified representation, which we prove to be NP-complete. Furthermore, we prove that finding a committee with justified representation and the highest approval voting score is NP-complete.

==> caption/CHANGELOG <==
caption package
===============

v1.0 (1994/10/27)
- 1st published version

v1.1 (1994/11/03)
- New option `centerlast'

v1.2 (1994/11/28)
- Support of the `float' package added

v1.3 (1995/01/09)
- Support of \captionlabelfont in subcaptions added

v1.4 (1995/01/30)
- New option `nooneline'

v2.0 (caption2, 1995/10/09)
- New experimental version with many new commands and features
- Support of the `longtable' package added

v2.1 (caption2, 2002/02/26)
- Adapted to version 2.1 of the subfigure package
- New options for interaction with other packages (float,...)
- New command \normalcaptionparams
- New commands \captionof and \captionof*
- New ifs \ifcaptionlabel and \ifignoreLTcapwidth
- \realcaptionwidth renamed to \captionlinewidth

v2.2 (caption2, 2007/04/06)
- Internal change: Uses the caption3 kernel now

v3.0 (2003/12/20)
- Completely rewritten in cooperation with Frank Mittelbach and Steven Cochran

v3.1 (2007/09/01)
- Improved compatibility to supported document classes and packages, but decreased compatibility to non-supported document classes and packages
- Support of the AMS & SMF document classes added
- Support of the `beamer' document class added
- Support of the `KOMA-Script' document classes added
- Support of the `floatflt' package added
- Support of the `fltpage' package added
- Support of the `picinpar' package added
- Support of the `picins' package added
- Support of the `threeparttable' package added
- Support of the `wrapfig' package added
- Support of the `xtab' package added
- Check against incompatible `ftcap' package added
- Check against incompatible `nonfloat' package added
- Check against incompatible `topcapt' package added
- Does not process global options anymore to avoid conflicts with document class options
- New option compatibility=
- New options font+=, labelfont+= & textfont+=
- New options hypcap= & hypcapspace=
- New options list= and listformat=
- New option options=
- New options figurewithin= and tablewithin=
- Starred variant of option margin*= added
- Starred variant of option style*= added
- Starred variant of option type*= added
- Font options `normal', `normalcolor', `color', `normalfont' & `stretch' added
- Default position changed from `bottom' to `auto'
- New command \DeclareFloatingEnvironment resp. \DeclareCaptionType
- New command \DeclareCaptionListFormat
- New command \captionlistentry
- Starred variant of \clearcaptionsetup added
- Optional argument added to \clearcaptionsetup
- Starred variant of \ContinuedFloat added
- \captionsetup{...} inside longtables added
- \captionsetup[singleline]{...} added
- A \label before \caption will result in warning "\label before \caption ignored"
- The counters lofdepth & lotdepth are supported now
- Label formats have three arguments now
- Optional argument added to \DeclareCaptionFormat; "format=plain" removed from single-line options of default format
- Caption label format `brace' added

v3.2 (2011/07/30)
- Support of `beamer' document class improved
- Support of `magyar' babel option added
- Support of `sansmath' package added
- Support of `titletoc' package added to \DeclareCaptionType & \DeclareCaptionSubType
- Support of `tocbasic' package added to \DeclareCaptionType
- New options calcmargin=, calcmargin*=, calcwidth=, and calcwidth*=
- New option listtype= added
- New option parboxrestore=partial/full
- New options within= & without
- Option slc= as abbreviation of singlelinecheck= added
- Pre-defined text format `empty' added
- New command \captionbox
- New command \phantomcaption
- New command \setcaptiontype as replacement for \captionsetup{type=...}
- New command \setcaptionsubtype as replacement for \captionsetup{subtype}
- "Hyperref support is turned off because hyperref has stopped early" is not a warning anymore but an information instead

v3.3 (2013/01/06)
- Revised handling of continued floats and sub-captions
- New option box= and appropriate command \DeclareCaptionBox
- New option list-entry= (see also endfloat package documentation)
- Support of multiple optional arguments added to \captionsetup (see bicaption package documentation)
- Adapted to the elsarticle document class
- Adapted to the current version of memhfixc package, provided by the memoir document class
- Fixed compatibility problem with breqn and nag packages
- Corrects incorrect load order hyperref-float now (needs hyperref v6.82q or newer)
- New switch \ifsinglelinecaption for usage inside own commands added


bicaption package
=================

v0.9 (2010/09/19)
- 1st published version (see also http://www.mrunix.de/forums/showthread.php?t=68312)

v1.0 (2011/09/03)
- Support for list entries added

v1.1 (2012/12/26)
- \captionmainlanguage and \selectcaptionlanguage added


ltcaption package
=================

v1.0 (2007/04/15)
- 1st version

v1.1 (2007/09/01)
- Adapted to the NTG document classes (Support of \CaptionLabelFont & \CaptionTextFont added)
- Adapted to the `floatrow' package by Olga Lapko
- New macro \LTcaptype
- New environment longtable*

v1.2 (2008/03/28)
- New skip \LTcapskip

v1.3 (2011/09/12)
- New macro \CaptionLabelSeparator


subcaption package
==================

v1.0 (2008/03/16)
- 1st published version

v1.1 (2011/08/17)
- New caption option subrefformat=
- New command \phantomsubcaption


newfloat package
================

v1.0 (2011/10/30)
- 1st published version

v1.1 (2013/04/27)
- New command \PrepareListOf


totalcount package
==================

v1.0 (2008/03/09)
- 1st published version



==> caption/README <==
==========================================================================

The `caption' package bundle
Copyright (C) 1994-2013 Axel Sommerfeldt (axel.sommerfeldt@f-m.fm)

License: LPPL = LaTeX Project Public Licence
Maintenance Status: maintained (by Axel Sommerfeldt)

Home page:
http://sourceforge.net/projects/latex-caption/

If you need help for installation please visit:
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=inst-miktex*
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=installthings
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=privinst

If you need help using these packages please visit:
http://www.latex-community.org/
http://tex.stackexchange.com/
http://www.mrunix.de/            (German)
http://www.golatex.de/           (German)

If you think you may have found a bug in these packages,
or want to report a suggestion for improvement, please visit:
http://sourceforge.net/p/latex-caption/tickets/

--------------------------------------------------------------------------

The `caption' package v3.3 offers customization of captions of floating
environments such `figure' and `table' and cooperates with the packages

  float, floatflt, fltpage, hyperref, hypcap, listings, longtable,
  picinpar, picins, rotating, sidecap, subfigure, supertabular,
  threeparttable, wrapfig, and xtab.

Furthermore the `floatrow', the `subcaption', and the `subfig' package
supports the `caption' package and uses its \captionsetup interface.

User Manual: caption-eng.pdf (English)
             caption-rus.pdf (Russian, outdated)
             caption-deu.pdf (German)

--------------------------------------------------------------------------

The `bicaption' package v1.1 is a tiny package supporting the typesetting
of bilingual captions.

User Manual: bicaption.pdf (English)

--------------------------------------------------------------------------

The `ltcaption' package v1.3 fixes caption problems with
other-than-center aligned longtables. (solving LaTeX PR `tools/3387')

A bonus feature is the addition of the environment longtable* which does
not increment the table counter.

This package will be loaded automatically by the `caption' package,
but can be used without the caption package, too.

User Manual: ltcaption.pdf (English)

--------------------------------------------------------------------------

The `subcaption' package v1.1 is a small package supporting typesetting
of sub-captions (by using the the sub-caption feature of the `caption'
package).

User Manual: subcaption.pdf (English)

--------------------------------------------------------------------------

The `newfloat' package v1.1 offers the command \DeclareFloatingEnvironment
for defining new floating environments which behave like the existing
floating environments "figure" and "table".

User Manual: newfloat.pdf (English)

==========================================================================
(The pictures cat.eps & elephant.eps were taken with permission from the
 LaTeX Companion examples.)


==> math/README <==
README for amsmath 2.14 [2013/01/14] American Mathematical Society

Copyright 2001-2004, 2007, 2008, 2010, 2011, 2013 American Mathematical Society.

This work may be distributed and/or modified under the
conditions of the LaTeX Project Public License, either version 1.3c
of this license or (at your option) any later version.
The latest version of this license is in
  http://www.latex-project.org/lppl.txt
and version 1.3c or later is part of all distributions of LaTeX
version 2005/12/01 or later.

This work has the LPPL maintenance status `maintained'.

The Current Maintainer of this work is the American Mathematical
Society.

American Mathematical Society
Technical Support
Publications Technical Group
201 Charles Street
Providence, RI 02904
USA
tel: (401) 455-4080
     (800) 321-4267 (USA and Canada only)
fax: (401) 331-3842
email: tech-support@ams.org

========================================================================
                               CONTENTS
I.   OVERVIEW
II.  INSTALLATION AND GETTING STARTED
III. SUBMITTING BUG REPORTS
IV.  REMARKS ON THIS RELEASE
V.   CHANGE LOG

========================================================================
I. OVERVIEW

The amsmath package is an extension package for LaTeX that provides
additional features to facilitate mathematical typesetting. It has been
developed by the American Mathematical Society and released for general
use as a service to the mathematical community. A number of smaller
auxiliary packages are also distributed with the amsmath package.

========================================================================
II. INSTALLATION AND GETTING STARTED

In order to use amsmath you need to have TeX installed first. TeX is
not an AMS product. For information on getting TeX see one of the
following:

    http://www.tug.org/
    http://www.ams.org/tex/tex-resources

If you are installing amsmath manually, see install.txt.

The primary documentation for amsmath is in

    amsldoc.pdf

Additional documentation files include:

    diffs-m.txt
    subeqn.pdf
    technote.pdf
    testmath.pdf

which are included in the collection.

========================================================================
III. SUBMITTING BUG REPORTS

Technical support is available via the addresses listed above.  Bug
reports should be submitted using the standard LaTeX bug reporting
system: Execute the command

    latex latexbug.tex

and follow the resulting instructions. Select "amslatex" when asked
for a category.

========================================================================
IV. REMARKS ON THIS RELEASE

Version 2.14 is a minor update to provide more fluid interoperability
with stix.sty.  It should be fully compatible with version 2.13.

========================================================================
V. CHANGE LOG (REVERSE CHRONOLOGICAL ORDER)

2013-01-14 amsmath.dtx 2.14

    * amsmath.sty 2.14
      -- Minimal changes to make amsmath compatible with stix.sty.

2000-07-18 amsmath.dtx 2.13
    -- After the numbering patches in 2.11, \notag failed in certain
       circumstances: introduce some more auxiliary functions to sort
       things out, and redefine \nonumber.

2000-06-29 amstext.dtx 2.01
    -- Use \f@size instead of \tf@size because they are not
       necessarily the same and the former is better for putting a few
       words into a display.

2000-06-06 amsmath.dtx 2.12
    -- Fix transposed lines in 2.11 patch.

2000-06-02 amsmath.dtx 2.11

    * amsmath.sty 2.11
      -- Prevent "Arithmetic overflow" error by guarding against
         divide-by-zero in \x@calc@shift@lc (align environment).

    * amsdtx.dtx
      -- Moved to the amscls distribution.

2000-05-25 amsmath.dtx 2.10
    -- Clear up error message for \allowdisplaybreaks[0].
    -- Make mathdisplay re-entrant by introducing mathdisplay@stack,
       to clear up numbering problems in unusual circumstances such as
       \[ \] nested inside minipage inside equation.

2000-04-21 amsmath.dtx 2.09
    -- Ensure good catcodes for " etc.

2000-03-16 amsmath.dtx 2.08
    -- Fixed erroneous tag placement on split with fleqn/tbtags options.

2000-03-15 amsmath.dtx 2.07
    -- Add \reset@strutbox@ to deal with the following bug: After
       $...\mbox{\Huge $...$}...$, line spacing is wrong in a
       following "gather" or other environment that uses \strut@.
    -- Patch to fix bug with intlimits option: too much space in the
       middle of \iint.
    -- Overhaul math accents again to fix a couple of bugs reported by
       Thimm.

2000-03-10 amsmath.dtx 2.06
    -- Change \MathAccent to \mathaccentV so \DeclareMathAccent won't
       give an error when redefining an accent.

2000-01-06 amsmath.dtx 2.05
    -- Fixed incorrect placement of fleqn/reqno equation numbers
       inside indented lists (displaywidth < columnwidth). Changed the
       multline/fleqn/leqno indent to match mathmargin when possible
       instead of always just using multlinetaggap.


==> subfig/README <==
Manifest and Documentation for the `subfig' package (version 1.3).
------------------------------------------------------------------------

This directory contains version 1.3 of the subfig package.  In a UNIX
or UNIX-like command shell, use `make' to extract the subfig package
and run the local tests.


MANIFEST:
---------
  The following files as well as the derivative files `subfig.sty' and
  `altsf.cfg' constitute the subfig package and are considered as "the
  work" under the LaTeX Project Public License (LPPL 1.3 or later).

Makefile           UNIX makefile to extract the subfig package
                       and related material.
README             This file.
subfig.dtx         The documented subfig package.
subfig.ins         The subfig package installation file.
subfig.pdf         The subfig package documentation (in PDF).
test1.tex          Test one: Basic checks and examples.
test2.tex          Test two: Check for extra space around figure
test3.tex          Test four: Test of optional args and \subref.
test4.tex          Test four: Test of interaction with hyperref.
test5.tex          Test five: Test of continued figures.
test6.tex          Test six: Test of options and option interaction.
test7.tex          Test seven: Test of class/package misuse of \let.


FILES AFTER `make':
-------------------
Makefile           UNIX makefile to extract the subfig package
                       and related material.
README             This file.
altsf.cfg          A subfig configuration file (which make the subfig 
                        package act similar to the subfigure package).
ltxdoc.cfg         Configuration file to print change history and
                       index on the subfig package documentation.       
subfig.dtx         The documented subfig package.
subfig.ins         The subfig package installation file.
subfig.pdf         The subfig package documentation (in PDF).
subfig.ps          The subfig package documentation (in PostScript).
subfig.sty         The subfig package 
test1.ps           Results of test one.
test1.tex          Test one: Basic checks and examples.
test2.ps           Results of test two.
test2.tex          Test two: Check for extra space around figure
test3.ps           Results of test three.
test3.tex          Test four: Test of optional args and \subref.
test4.pdf          Results of test four.
test4.tex          Test four: Test of interaction with hyperref.
test5.ps           Results of test five.
test5.tex          Test five: Test of continued figures.
test6.ps           Results of test six.
test6.tex          Test six: Test of options and option interaction.
test7.tex          Test seven: Test of class/package misuse of \let.
test7a.ps          Log from test seven run.
test7b.ps          Results of test seven.


NOTES:
------

1. To verify the results of the test(s) (which are run using the
   preferred options), compare with the test(s) found at:
   http://www.cs.cmu.edu/~sdc/latex/subfig.13/

2. This version of the subfig package removes a "feature" which
   allowed a line break to occur between two subfloats separated
   by whitespace instead of requiring an explicit "\\".  If this
   "feature" was used to position sub-floats, they may now be
   incorrectly displayed.

   If this occurs, the solution is to add an expicit linebreak
   between the problem sub-floats.  For example, the following
   to the left would seem to work correctly, but suppressed
   the "farskip" placing the figures too close together and 
   will, now, no longer work.  It should be written as on the
   left.

   \begin{figure}                  \begin{figure}		
     \centering	                     \centering		
       \subfloat[One.]{...}%	       \subfloat[One.]{...}	
     \hspace{.25in}%		     \hspace{.25in}%		
       \subfloat[Two.]{...}	       \subfloat[Two.]{...} \\	
       \subfloat[Three.]{...}%         \subfloat[Three.]{...}	
     \hspace{.25in}%		     \hspace{.25in}%		
       \subfloat[Four.]{...}%	       \subfloat[Four.]{...}	
     \caption{Simple Case.}	     \caption{Simple Case.}	
   \end{figure}                    \end{figure}               











==> xcolor.sty.tex <==
%%
%% This is file `xcolor.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xcolor.dtx  (with options: `package')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from xcolor.sty.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file xcolor.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%%
%% ---------------------------------------------------------
%% Copyright (C) 2003-2004 by Dr. Uwe Kern <xcolor@ukern.de>
%% ---------------------------------------------------------
%%
%% Please send error reports and suggestions for
%% improvements to the above email address.
%%
%% This package contains code copied from
%%
%% color.dtx [1999/02/16 v1.0i Standard LaTeX Color (DPC)]
%% Copyright (C) 1994--1999 David Carlisle
%%
%% which is part of the Standard LaTeX `Graphics Bundle'.
%%
\def\XCfilesource{xcolor.dtx}%
\def\XCfileversion{v2.00}%
\def\XCfiledate{2004/07/04}%
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{xcolor}[\XCfiledate\space\XCfileversion\space
                         LaTeX color extensions (UK)]
\edef\XC@catcodes
 {\catcode`\noexpand\!\the\catcode`\!\relax
  \catcode`\noexpand\:\the\catcode`\:\relax
  \catcode`\noexpand\-\the\catcode`\-\relax
  \catcode`\noexpand\+\the\catcode`\+\relax
  \catcode`\noexpand\;\the\catcode`\;\relax
  \catcode`\noexpand\"\the\catcode`\"\relax
  \catcode`\noexpand\^^A\the\catcode`\^^A\relax}
\catcode`\!=12
\catcode`\:=12
\catcode`\-=12
\catcode`\+=12
\catcode`\;=12
\catcode`\"=12
\catcode`\^^A=\catcode`\%
\newif\ifcolors@ \colors@true
\newif\ifcolorerrors@
\newif\ifglobalcolors \globalcolorsfalse
\newif\ifconvertcolorsD
\newif\ifconvertcolorsU
\newif\ifblendcolors
\newif\ifmaskcolors
\newif\ifXC@@tst
\def\c@lor@error#1%
 {\ifcolorerrors@\PackageError{xcolor}{Undefined color #1}\@ehc
  \else\PackageWarning{xcolor}{Undefined color #1}\fi}
\def\XC@append#1#2%
 {\ifx#1\@undefined\def#1{#2}\else\ifx#1\relax\def#1{#2}\else
  \toks@\expandafter{#1#2}\edef#1{\the\toks@}\fi\fi}
\def\selectcolormodel#1%
 {\@ifundefined{XC@mod@#1}%
   {\c@lor@error{model `#1'}}%
   {\expandafter\ifx\csname XC@mod@#1\endcsname\XC@mod@natural
      \def\XC@tgt@mod##1{##1}\convertcolorsDfalse\convertcolorsUfalse
    \else
      \edef\XC@tgt@mod##1{#1}\convertcolorsDtrue\convertcolorsUtrue
    \fi}}
\def\XC@mod@named{named}
\@tfor\@@tmp:={natural}{rgb}{cmy}{cmyk}{hsb}{gray}{RGB}{HTML}{HSB}{Gray}\do
 {\expandafter\let\csname XC@mod@\@@tmp\endcsname\@@tmp
  \edef\@@tmp
   {\noexpand\DeclareOption{\@@tmp}{\noexpand\selectcolormodel{\@@tmp}}}%
  \@@tmp}
\DeclareOption{monochrome}
 {\ExecuteOptions{hideerrors}%
  \AtEndOfPackage
   {\colors@false
    \def\set@color{\c@lor@special\m@ne
      {color push \current@color}\aftergroup\reset@color}%
    \def\reset@color{\c@lor@special\m@ne{color pop}}%
    \def\set@page@color{\c@lor@special\m@ne{background \current@color}}}}
\let\XC@colornames\relax
\DeclareOption{dvipsnames}{\XC@append\XC@colornames{\input{dvipsnam.def}}}
\DeclareOption{svgnames}{\XC@append\XC@colornames{\input{svgnam.def}}}
\DeclareOption{pst}{\def\XC@pst{\RequirePackage{pstcol}}}
\DeclareOption{table}{\def\XC@table{\RequirePackage{colortbl}}}
\DeclareOption{hyperref}
 {\@tfor\@@tmp:={cite}{file}{link}{menu}{page}{run}{url}\do
   {\expandafter\edef\csname KV@Hyp@x\@@tmp bordercolor\endcsname #1%
     {\noexpand\XC@bordercolor{\@@tmp}{#1}}}%
  \AtEndOfPackage
   {\GetGinDriver\def\KV@Hyp@xpdfborder#1{\edef\@pdfborder{#1}}%
    \@tfor\@@tmp:={dvips}\do
     {\ifx\GinDriver\@@tmp
       \def\KV@Hyp@xpdfborder#1%
        {\edef\@pdfborder{#1}\expandafter\XC@pdfborder\@pdfborder\relax}%
      \@break@tfor\fi}}}
\providecommand\Gin@driver{}
\@tfor\@@tmp:={dvipdf}{dvipdfm}{dvips}{dvipsone}{dviwin}{emtex}%
              {pctex32}{pctexhp}{pctexps}{pctexwin}{pdftex}{tcidvi}%
              {textures}{truetex}{vtex}\do
 {\edef\@@tmp{\noexpand\DeclareOption{\@@tmp}%
    {\noexpand\def\noexpand\Gin@driver{\@@tmp.def}}}%
  \@@tmp}
\DeclareOption{dviwindo}{\ExecuteOptions{dvipsone}}
\DeclareOption{oztex}{\ExecuteOptions{dvips}}
\DeclareOption{xdvi}{\ExecuteOptions{dvips,monochrome}}
\DeclareOption{showerrors}{\colorerrors@true}
\DeclareOption{hideerrors}{\colorerrors@false}
\DeclareOption{debugshow}{\catcode`\^^A=9 \let\GDebug\typeout}
\DeclareOption*%
 {\PackageInfo{xcolor}{Package option `\CurrentOption' ignored}}
\ExecuteOptions{natural,showerrors}
\InputIfFileExists{color.cfg}{}{}
\ProcessOptions\relax
\if!\Gin@driver!
  \PackageError{xcolor}
    {No driver specified}
    {You should make a default driver option in a file \MessageBreak
     color.cfg\MessageBreak
     eg: \protect\ExecuteOptions{dvips}}
\else
  \PackageInfo{xcolor}{Driver file: \Gin@driver}
  \@ifundefined{ver@\Gin@driver}{\input{\Gin@driver}}{}
\fi
\@nameuse{XC@pst}
\@namedef{ver@color.sty}{1999/02/16}
\@nameuse{XC@table}
\long\def\@secondoffive#1#2#3#4#5{#2}
\def\@namelet#1#2%
 {\expandafter\let\csname#1\expandafter\endcsname\csname#2\endcsname}
\def\@namexdef#1{\expandafter\xdef\csname #1\endcsname}
\def\aftergroupdef#1#2%
 {\edef\@@tmp{\noexpand\def\noexpand#1{#2}}%
  \expandafter\endgroup\@@tmp}
\begingroup
\catcode`\!=13 \catcode`\:=13 \catcode`\-=13 \catcode`\+=13
\catcode`\;=13 \catcode`\"=13
\gdef\XC@edef#1#2%
 {\begingroup
  \ifnum\catcode`\!=13 \edef!{\string!}\fi
  \ifnum\catcode`\:=13 \edef:{\string:}\fi
  \ifnum\catcode`\-=13 \edef-{\string-}\fi
  \ifnum\catcode`\+=13 \edef+{\string+}\fi
  \ifnum\catcode`\;=13 \edef;{\string;}\fi
  \ifnum\catcode`\"=13 \edef"{\string"}\fi
  \edef\@@tmp{#2}\@onelevel@sanitize\@@tmp
  \aftergroupdef#1\@@tmp}
\endgroup
\def\@ifxempty#1{\@@ifxempty#1\@@ifxempty\XC@@}
\def\@@ifxempty#1#2\XC@@
 {\ifx#1\@@ifxempty
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}
\def\xglobal{\xglobal@stop\begingroup\futurelet\@@tok\xglobal@test}
\def\xglobal@test
 {\expandafter\@tfor\expandafter\@@tmp
   \expandafter:\expandafter=\xglobal@list\do
    {\expandafter\ifx\@@tmp\@@tok
       \aftergroup\let\aftergroup\xglobal@\@break@tfor\fi}%
  \endgroup\global}
\def\xglobal@stop{\let\xglobal@\@empty}
\xglobal@stop
\def\xglobal@list
 {\definecolor\providecolor\colorlet\definecolorset\providecolorset
  \blendcolors\maskcolors}
\def\xglobalize@#1{\ifx\xglobal@\global\global\let#1#1\fi}
\def\GetGinDriver{\expandafter\GetGinDriver@\Gin@driver.:}
\def\GetGinDriver@#1.#2:%
 {\def\GinDriver{#1}\@tempswatrue
  \@tfor\@@tmp:={dvips}{pdftex}{dvipdf}{dvipdfm}{dvipsone}{vtex}{textures}%
  \do{\ifx\GinDriver\@@tmp\@tempswafalse\@break@tfor\fi}%
  \if@tempswa\def\GinDriver{hypertex}\fi}
\def\@hex@Hex#1{\ifx#1\relax\else\expandafter\@hex@@Hex\expandafter#1\fi}
\def\@hex@@Hex#1%
 {\if#1aA\else \if#1bB\else \if#1cC\else \if#1dD\else \if#1eE\else
  \if#1fF\else #1\fi\fi\fi\fi\fi\fi \@hex@Hex}
\def\rdivide#1#2%
 {\begingroup\toks@{#1}\edef\@@tmp{\noexpand\@tempdima\the#1}%
  \@defaultunits\@tempdimb=#2pt\relax\@nnil \@@tmp\relax
  \ifdim\@tempdima<\z@ \@tempdima-\@tempdima\def\@sign{-}\else
    \def\@sign{}\fi
  \ifdim\@tempdimb<\z@ \@tempdimb-\@tempdimb\edef\@sign{\@sign-}\fi
  \ifdim\@tempdima<.1\maxdimen \ifdim\@tempdimb<.01\maxdimen
    \lshift\@tempdima \lshift\@tempdimb \fi\fi
  \@tempcnta=\@tempdima \@tempcntb=\@tempdimb
  \count@=\@tempcnta \divide\count@\@tempcntb
  \edef\@@tmp{\number\count@.}%
  \@tempswatrue  \@rdivide \@rdivide \@rdivide \@rdivide \@rdivide
  \@tempswafalse \@rdivide
  \dimen@\@@tmp\p@ \ifnum\count@>4\advance\dimen@.00001\p@\fi
  \dimen@\@sign\dimen@
  \edef\@@tmp{\the\toks@\the\dimen@}%
  \expandafter\endgroup\@@tmp}
\def\@rdivide
 {\multiply\count@\@tempcntb \advance\@tempcnta-\count@
  \multiply\@tempcnta10 \count@=\@tempcnta \divide\count@\@tempcntb
  \if@tempswa\edef\@@tmp{\@@tmp\number\count@}\fi}
\def\rmultiply#1#2%
 {\begingroup
  \edef\@@mul{#2}\@tempdima\the#1\relax
  \afterassignment\@tempdimb\@tempcntb=\@@mul\p@
  \ifdim\@tempdima<\z@ \@tempdima-\@tempdima\def\@sign{-}\else
    \def\@sign{}\fi
  \ifnum\@tempcntb<\z@ \@tempcntb-\@tempcntb\edef\@sign{\@sign-}\fi
  \lshift\@tempdima \dimen@\z@
  \expandafter\@rmultiply\@@mul.0.\@nil
  \advance\dimen@\@tempcntb\@tempdima \rshift\dimen@
  \dimen@\@sign\dimen@
  \edef\@@tmp{#1\the\dimen@}%
  \expandafter\endgroup\@@tmp}
\def\@rmultiply#1.#2.#3\@nil
 {\def\@@tmp{}%
  \@tfor\@@mul:=#2\do
   {\edef\@@tmp
     {\advance\dimen@\@@mul\@tempdima \divide\dimen@10 \@@tmp}}%
  \@@tmp}
\def\lshift#1{#1\expandafter\lshift@\the#1}
\def\llshift#1{\lshift#1\lshift#1}
\def\lshiftnum#1{\expandafter\lshiftnum@#1.00.:}
\def\lshiftnum@#1.#2#3.#4:{#1#2\ifnum0#3>\z@.#3\fi}
\def\llshiftnum#1{\expandafter\llshiftnum@#1\@empty.00.:}
\def\llshiftnum@#1.#2#3#4.#5:%
 {#1#2\ifnum0#3>\z@#3\else0\fi\ifnum0#4>\z@.#4\fi}
\def\lshiftset#1#2{\edef\@@XC{\noexpand\lshiftnum{#2}}#1\@@XC\p@}
\def\llshiftset#1#2{\edef\@@XC{\noexpand\llshiftnum{#2}}#1\@@XC\p@}
\def\rshift#1{#1\expandafter\rshift@\the#1}
\def\rrshift#1{\rshift#1\rshift#1}
\begingroup
\catcode`P=12
\catcode`T=12
\lowercase
 {\def\@@tmp{\def\lshift@##1.##2##3PT{##1##2\ifnum0##3>\z@.##3\fi\p@}
             \def\rshift@##1.##2PT{\rshift@@##1\relax##2\p@}}}
\expandafter\endgroup\@@tmp
\def\rshift@@#1#2%
 {\ifx#2\relax.#1\else#1\expandafter\rshift@@\expandafter#2\fi}
\def\XC@inflate#1#2#3#4%
 {\edef#4{#2,\ifx#1\XC@mod@cmyk #3\else
             \ifx#1\XC@mod@gray ,,,#3,,,\else ,#3,\fi\fi}}
\def\XC@vec#1,#2,#3,#4,#5,#6,#7,#8,#9%
 {\def\@@tmp{}%
  \XC@vec@{#1}{#5}%
  \@ifxempty{#2}{}%
   {\XC@vec@{#2}{#6}\XC@vec@{#3}{#7}\@ifxempty{#4}{}{\XC@vec@{#4}{#8}}}%
  \aftergroupdef#9\@@tmp}
\def\XC@add{\begingroup \let\XC@vec@\XC@add@ \XC@vec}
\def\XC@add@#1#2%
 {\llshiftset\dimen@{#1}\llshiftset\@tempdima{#2}%
  \advance\dimen@\@tempdima \rrshift\dimen@
  \edef\@@tmp{\ifx\@@tmp\@empty\else\@@tmp,\fi\strip@pt\dimen@}}
\def\XC@sub{\begingroup \let\XC@vec@\XC@sub@ \XC@vec}
\def\XC@sub@#1#2{\XC@add@{#1}{-#2}}
\def\XC@mul{\begingroup \let\XC@vec@\XC@mul@ \XC@vec}
\def\XC@mul@#1#2%
 {\llshiftset\dimen@{#1}\rmultiply\dimen@{#2}\rrshift\dimen@
  \edef\@@tmp{\ifx\@@tmp\@empty\else\@@tmp,\fi\strip@pt\dimen@}}
\def\XC@mix%
 {\begingroup
  \@tempdima\dimen@ \@tempdimb100\p@ \advance\@tempdimb-\@tempdima
  \let\XC@vec@\XC@mix@ \XC@vec}
\def\XC@mix@#1#2%
 {\dimen@#1\@tempdima \advance\dimen@#2\@tempdimb \rrshift\dimen@
  \edef\@@tmp{\ifx\@@tmp\@empty\else\@@tmp,\fi\strip@pt\dimen@}}
\def\XC@calc@#1,#2,#3,#4,#5:#6%
 {\toks@\expandafter{\csname XC@calc#6\endcsname}%
  \the\toks@{#1}\@@tmp
  \@ifxempty{#2}{}%
   {\the\toks@{#2}\@tempa \the\toks@{#3}\@tempb
    \@ifxempty{#4}%
     {\edef\@@tmp{\@@tmp,\@tempa,\@tempb}}%
     {\the\toks@{#4}\@tempc \edef\@@tmp{\@@tmp,\@tempa,\@tempb,\@tempc}}}}
\def\XC@calcC#1#2%
 {\lshiftset\dimen@{-#1}\advance\dimen@10\p@ \rshift\dimen@
  \edef#2{\strip@pt\dimen@}}
\def\XC@calcD#1#2%
 {\dimen@#1\p@ \rdivide\dimen@\@@scl \edef#2{\strip@pt\dimen@}}
\def\XC@calcH#1#2%
 {\count@#1 \divide\count@\sixt@@n \edef\XC@@tmp{\hexnumber@\count@}%
  \multiply\count@-\sixt@@n \advance\count@#1
  \edef#2{\XC@@tmp\hexnumber@\count@}}
\def\XC@calcM#1#2%
 {\dimen@#1\p@ \dimen@\@@scl\dimen@ \advance\dimen@.5\p@
  \afterassignment\dimen@\count@=\the\dimen@ \edef#2{\number\count@}}
\def\XC@calcN#1#2%
 {\edef#2{#1}%
  \edef#2{\ifdim#2\p@<\z@0\else \ifdim#2\p@<\p@
          0\expandafter\XC@@calcN#2.0.:\else 1\fi\fi}}
\def\XC@@calcN#1.#2.#3:%
 {\ifnum0#2=0 \else.\XC@@@calcN#2:\fi}
\def\XC@@@calcN#1#2:%
 {\ifnum0#1#2=0 \else #1\ifnum0#2=0 \else \XC@@@calcN#2:\fi\fi}
\def\XC@calcS#1#2%
 {\lshiftset\dimen@{#1}\dimen@\lshiftnum\@@scl\dimen@ \rrshift\dimen@
  \edef#2{\strip@pt\dimen@}}
\def\XC@calcT#1#2%
 {\lshiftset\dimen@{#1}\advance\dimen@\lshiftnum\@@arg\p@ \rshift\dimen@
  \edef#2%
   {\ifdim\dimen@>\p@1\else\ifdim\dimen@<\z@0\else\strip@pt\dimen@\fi\fi}}
\def\XC@calcU#1#2%
 {\dimen@#1\p@
  \ifdim\dimen@=\p@\else
    \afterassignment\dimen@\count@=\the\dimen@
    \ifnum\count@<\z@
      \lshift\dimen@ \dimen@-\dimen@ \advance\dimen@10\p@ \rshift\dimen@
    \fi
  \fi
  \edef#2{\strip@pt\dimen@}}
\ifx\rangeRGB\@undefined\def\rangeRGB{255}\fi
\ifx\rangeHSB\@undefined\def\rangeHSB{240}\fi
\ifx\rangeGray\@undefined\def\rangeGray{15}\fi
\ifx\adjustUCRBG\@undefined\def\adjustUCRBG{1,1,1,1}\fi
\ifx\colorseriescycle\@undefined\def\colorseriescycle{16}\fi
\def\XC@clr@rgb@white{,,}
\def\XC@clr@cmy@white{0,0,0}
\def\XC@clr@cmyk@white{0,0,0,0}
\def\XC@clr@hsb@white{\@@hue,0,}
\def\XC@clr@hsb@gray{\@@hue,0,.5}
\def\XC@clr@hsb@black{\@@hue,0,0}
\def\XC@clr@gray@white{}
\@tfor\@@tmp:={grad}{last}{step}\do
 {\@namelet{XC@met@\@@tmp}{@@tmp}}
\def\definecolor{\@testopt{\XC@definecolor}{}}
\def\XC@definecolor[#1]#2#3#4%
 {\@ifundefined{XC@mod@#3}%
   {\c@lor@error{model `#3'}}%
   {\begingroup
    \edef\@@cls{#1}\XC@edef\@@nam{#2}\edef\@@mod{#3}\XC@edef\@@clr{#4}%
    \XC@logdef\@@nam
    \ifx\@@mod\XC@mod@named
      \XC@@colorlet\@@nam\@@clr
    \else
      \ifconvertcolorsD
        \edef\@@mod{\XC@tgt@mod{#3}}\convertcolorspec{#3}\@@clr\@@mod\@@clr
      \fi
      \XC@coremodel\@@mod\@@clr
      \csname color@\@@mod\expandafter\endcsname
        \expandafter\@@drv\expandafter{\@@clr}%
      \ifx\@@cls\@empty
        \@temptokena{}%
      \else
        \@nameuse{define@color@\@@cls}{\@@nam}\@@drv
        \@temptokena\expandafter{\@@col}%
        \csname color@\@@cls\expandafter\endcsname
          \expandafter\@@drv\expandafter{\@@nam}%
      \fi
      \toks@\expandafter{\@@drv}%
      \edef\@@tmp
       {\ifglobalcolors\global\else\xglobal@\fi
        \noexpand\@namedef{\string\color@\@@nam}%
         {\noexpand\xcolor@{\the\@temptokena}{\the\toks@}{\@@mod}{\@@clr}}}%
    \fi
    \expandafter\endgroup\@@tmp\xglobal@stop}}
\let\xdefinecolor\definecolor
\def\providecolor{\@testopt{\XC@providecolor}{}}
\def\XC@providecolor[#1]#2#3#4%
 {\XC@edef\XC@@tmp{#2}%
  \@ifundefined{\string\color@\XC@@tmp}{\definecolor[#1]{#2}{#3}{#4}}%
   {\ifnum\XC@tracing>0
      \PackageInfo{xcolor}{Ignoring color definition `\XC@@tmp'}\fi}}
\def\xcolor@#1#2#3#4{#2}
\def\colorlet#1{\@testopt{\XC@colorlet{#1}}{}}
\def\XC@colorlet#1[#2]#3%
 {\begingroup
  \XC@edef\@@nam{#1}\edef\@@mod{#2}\XC@edef\@@tmp{#3}\XC@@tsttrue
  \@ifundefined{\string\color@\@@tmp}%
    {}{\ifx\@@mod\@empty\XC@@tstfalse\fi}%
  \ifXC@@tst
    \extractcolorspec\@@tmp\@@tmp
    \ifx\@@mod\@empty\else
      \expandafter\convertcolorspec\@@tmp\@@mod\@@tmp
      \edef\@@tmp{{\@@mod}{\@@tmp}}\fi
    \edef\@@tmp{\noexpand\XC@definecolor[]{\@@nam}\@@tmp}%
  \else
    \XC@logdef\@@nam\XC@@colorlet\@@nam\@@tmp
  \fi
  \expandafter\endgroup\@@tmp\xglobal@stop}
\def\XC@@colorlet#1#2%
 {\@ifundefined{\string\color@#2}%
   {\c@lor@error{`#2'}\let\@@tmp\@empty}%
   {\edef\@@tmp
     {\ifglobalcolors\global\else\xglobal@\fi
      \noexpand\@namelet{\string\color@#1}{\string\color@#2}}}}
\def\DefineNamedColor#1{\XC@definecolor[#1]}
\def\definecolorset
 {\let\XC@defclr\definecolor\@testopt{\XC@definecolorset}{}}
\def\XC@definecolorset[#1]#2#3#4#5%
 {\XC@edef\XC@@tmp{#5}\let\XC@@glb\xglobal@
  \def\XC@@definecolorset##1,##2;%
   {\@ifxempty{##1}{}%
     {\let\xglobal@\XC@@glb
      \XC@defclr[#1]{#3##1#4}{#2}{##2}\XC@@definecolorset}}%
  \expandafter\XC@@definecolorset\XC@@tmp;,;}
\def\providecolorset
 {\let\XC@defclr\providecolor\@testopt{\XC@definecolorset}{}}
\def\definecolorseries#1#2#3%
 {\@testopt{\XC@definecolorseries{#1}{#2}{#3}}{}}
\def\XC@definecolorseries#1#2#3[#4]#5%
 {\@testopt{\XC@@definecolorseries{#1}{#2}{#3}[#4]{#5}}{}}
\def\XC@@definecolorseries#1#2#3[#4]#5[#6]#7%
 {\begingroup
  \edef\@@mod{#2}%
  \@ifxempty{#4}{\extractcolorspec{#5}\@@clr}{\edef\@@clr{{#4}{#5}}}%
  \expandafter\convertcolorspec\@@clr\@@mod\@@clr
  \@namexdef{\string\colorB@#1}{{\@@mod}{\@@clr}}%
  \edef\@@met{#3}%
  \ifx\@@met\XC@met@last
    \@ifxempty{#6}{\extractcolorspec{#7}\@@tmp}{\edef\@@tmp{{#6}{#7}}}%
    \expandafter\convertcolorspec\@@tmp\@@mod\@@tmp
    \XC@inflate\@@mod\@@tmp\@@clr\@@tmp
    \expandafter\XC@sub\@@tmp,\@@tmp
  \else
    \edef\@@tmp{#7}%
  \fi
  \@namexdef{\string\colorD@#1}{{\@@met}{\@@tmp}}%
  \endgroup}
\def\resetcolorseries{\@testopt{\XC@resetcolorseries}{}}
\def\XC@resetcolorseries[#1]#2%
 {\begingroup
  \@namexdef
   {\string\color@#2}{\noexpand\xcolor@{}{}\@nameuse{\string\colorB@#2}}%
  \@namelet{@@tmp}{\string\colorD@#2}%
  \edef\@@met{\expandafter\@firstoftwo\@@tmp}%
  \edef\@@tmp{\expandafter\@secondoftwo\@@tmp}%
  \ifx\@@met\XC@met@step\else
    \edef\@@scl{\@ifxempty{#1}\colorseriescycle{#1}}%
    \expandafter\XC@calc@\@@tmp,,,,:D%
  \fi
  \@namexdef{\string\colorS@#2}{\@@tmp}%
  \endgroup}
\def\XC@step#1%
 {\let\xcolor@\@gobbletwo\edef\@@tmp{\@nameuse{\string\color@#1}}%
  \expandafter\XC@@step\@@tmp{#1}%
  \@namexdef{\string\color@#1}{\noexpand\xcolor@{}{}{\@@mod}{\@@tmp}}}
\def\XC@@step#1#2#3%
 {\def\@@mod{#1}\def\@@tmp{#2}\edef\@@vec{\@nameuse{\string\colorS@#3}}%
  \@whilenum\@tempcnta>\z@\do
   {\XC@inflate\@@mod\@@tmp\@@vec\@@tmp
    \expandafter\XC@add\@@tmp,\@@tmp \expandafter\XC@calc@\@@tmp,,,,:U%
    \advance\@tempcnta\m@ne}}
\def\XC@stepabs#1%
 {\edef\@@tmp{\@nameuse{\string\colorB@#1}}%
  \expandafter\XC@@step\@@tmp{#1}%
  \edef\@@tmp
   {\noexpand\def\noexpand\@@mod{\@@mod}%
    \noexpand\def\noexpand\@@clr{\@@tmp}}}
\def\blendcolors{\@ifstar{\XC@blendcolors\colorblend}{\XC@blendcolors{}}}
\def\XC@blendcolors#1#2%
 {\edef\colorblend{#1}\XC@edef\XC@@tmp{#2}%
  \ifx\XC@@tmp\@empty
    \xglobal@\blendcolorsfalse
  \else
    \xglobal@\blendcolorstrue
    \expandafter\XC@@blendcolors\XC@@tmp!!\@nil
  \fi
  \xglobalize@\colorblend \xglobal@stop}
\def\XC@@blendcolors!#1!#2!#3\@nil
 {\@ifxempty{#1}{}%
   {\@ifxempty{#2}%
    {\edef\colorblend{\colorblend!#1!white}}%
    {\edef\colorblend{\colorblend!#1!#2}\XC@@blendcolors!#3!\@nil}}}
\blendcolors{}
\def\maskcolors{\@testopt{\XC@maskcolors}{}}
\def\XC@maskcolors[#1]#2%
 {\XC@edef\colormask{#2}%
  \ifx\colormask\@empty
    \xglobal@\maskcolorsfalse \def\XC@mmod{}\def\XC@mclr{}%
  \else
    \xglobal@\maskcolorstrue \extractcolorspec\colormask\XC@mclr
    \edef\XC@mmod{\expandafter\@firstoftwo\XC@mclr}%
    \edef\XC@mclr{\expandafter\@secondoftwo\XC@mclr}%
    \@ifxempty{#1}{}%
     {\convertcolorspec\XC@mmod\XC@mclr{#1}\XC@mclr \edef\XC@mmod{#1}}%
    \XC@coremodel\XC@mmod\XC@mclr
  \fi
  \xglobalize@\colormask \xglobalize@\XC@mmod \xglobalize@\XC@mclr
  \xglobal@stop}
\maskcolors{}
\DeclareRobustCommand\color
 {\@ifnextchar[\@undeclaredcolor\@declaredcolor}
\def\@undeclaredcolor[#1]#2%
 {\begingroup
  \edef\@@mod{#1}\XC@edef\@@clr{#2}%
  \ifblendcolors
    \ifx\colorblend\@empty\else
      \edef\@@mix{\expandafter\@gobble\colorblend}\@tempswafalse
      \XC@coremodel\@@mod\@@clr\@xcolor@{}{}\@@mod\@@clr
    \fi
  \fi
  \ifconvertcolorsU
    \edef\@@tmp{\XC@tgt@mod{\@@mod}}%
    \convertcolorspec\@@mod\@@clr\@@tmp\@@clr \let\@@mod\@@tmp
  \fi
  \ifmaskcolors
    \convertcolorspec\@@mod\@@clr\XC@mmod\@@clr
    \let\@@mod\XC@mmod
    \XC@inflate\@@mod\XC@mclr\@@clr\@@tmp
    \expandafter\XC@mul\@@tmp,\@@clr
  \fi
  \edef\@@tmp{\noexpand\XC@undeclaredcolor{\@@mod}{\@@clr}}%
  \expandafter\endgroup\@@tmp}
\def\XC@undeclaredcolor#1#2%
 {\@ifundefined{color@#1}%
   {\c@lor@error{model `#1'}}%
   {\@nameuse{color@#1}\current@color{#2}%
    \edef\XC@current@color{\noexpand\xcolor@{}{\current@color}{#1}{#2}}%
    \XC@display}}
\def\@declaredcolor#1%
 {\XC@edef\XC@@tmp{#1}\XC@@tstfalse
  \ifcase\XC@type{\XC@@tmp}\relax \XC@@tsttrue\or \relax\else
    \ifblendcolors\XC@@tsttrue\fi \ifmaskcolors\XC@@tsttrue\fi
    \ifconvertcolorsU\XC@@tsttrue\fi
  \fi
  \ifXC@@tst
    \expandafter\XC@declaredcolor
  \else
    \expandafter\XC@@declaredcolor
  \fi}
\def\XC@declaredcolor
 {\XC@split\XC@@tmp
  \edef\@@tmp{\noexpand\@undeclaredcolor[\@@mod]{\@@clr}}%
  \expandafter\endgroup\@@tmp}
\def\XC@@declaredcolor
 {\@namelet{XC@current@color}{\string\color@\XC@@tmp}%
  \edef\current@color{\XC@current@color}%
  \XC@display}
\def\@xcolor@#1#2#3#4%
 {\edef\@@mod{#3}\edef\@@clr{#4}%
  \ifx\@@mix\@empty\else\expandafter\@xcolor@@\@@mix!!!!\@nil\fi
  \if@tempswa
    \@namelet{@@tmp}{XC@cnv@\@@mod @compl}%
    \ifx\@@tmp\relax \expandafter\XC@calc@\@@clr,,,,:C\else
                     \expandafter\@@tmp\@@clr,\fi
    \let\@@clr\@@tmp
  \fi}
\def\@xcolor@@#1!#2!#3!#4!#5\@nil
 {\dimen@\@ifxempty{#1}{100}{#1}\p@
  \edef\@@mix{\@ifxempty{#2}{white}{#2}}%
  \ifdim\dimen@=100\p@
    \expandafter\XC@postfix\@@mix]\relax
  \else\ifdim\dimen@=\z@
    \extractcolorspec\@@mix\@@tmp
    \edef\@@mod{\expandafter\@firstoftwo\@@tmp}%
    \edef\@@clr{\expandafter\@secondoftwo\@@tmp}%
  \else
    \@namelet{@@tmp}{XC@clr@\@@mod @\@@mix}%
    \ifx\@@tmp\relax
      \extractcolorspec\@@mix\@@tmp
      \ifx\@@mod\XC@mod@gray
        \edef\@@mod{\expandafter\@firstoftwo\@@tmp}%
          \edef\@@tmp{\expandafter\@secondoftwo\@@tmp}%
          \convertcolorspec\XC@mod@gray\@@clr\@@mod\@@clr
      \else
        \expandafter\convertcolorspec\@@tmp\@@mod\@@tmp
      \fi
    \else
      \ifx\@@mod\XC@mod@hsb\expandafter\XC@extract@hue\@@clr:\@@hue\fi
    \fi
    \XC@inflate\@@mod\@@clr\@@tmp\@@tmp
    \expandafter\XC@mix\@@tmp,\@@clr
  \fi\fi
  \@ifxempty{#3}%
   {\@ifxempty{#4}{}{\@xcolor@@!#4!#5\@nil}}%
   {\@xcolor@@#3!#4!#5\@nil}}
\def\XC@split#1%
 {\begingroup\XC@edef\@@tmp{#1}\expandafter\XC@split@i\@@tmp:\@nil}
\def\XC@split@i#1:#2\@nil
 {\@ifxempty{#2}{\XC@split@v}{\XC@split@ii#1,,:#2}}
\def\XC@split@ii#1,#2,#3:#4:%
 {\edef\XC@@mod{\@nameuse{XC@mod@#1}}\let\@tempa\@empty
  \@ifxempty{#2}{\XC@@tsttrue\@tempdima\z@}{\XC@@tstfalse\@tempdima#2\p@}%
  \XC@split@iii#4;,;}
\def\XC@split@iii#1,#2;%
 {\@ifxempty{#1}%
   {\let\XC@@clr\@empty \@tempa \expandafter\XC@calc@\XC@@clr,,,,:U%
    \let\@@mod\XC@@mod \let\@@clr\@@tmp}
   {\XC@append\@tempa{\XC@split@iv{#1}{#2}}%
    \ifXC@@tst\advance\@tempdima#2\p@\fi
    \XC@split@iii}}
\def\XC@split@iv#1#2%
 {\def\@@tmp{#1}\XC@split@v
  \ifx\@@mod\XC@@mod\else
    \convertcolorspec\@@mod\@@clr\XC@@mod\@@clr
  \fi
  \dimen@#2\p@ \rdivide\dimen@\@tempdima
  \edef\@@scl{\strip@pt\dimen@}%
  \expandafter\XC@calc@\@@clr,,,,:S%
  \ifx\XC@@clr\@empty\let\XC@@clr\@@tmp\else
    \XC@inflate\XC@@mod\XC@@clr\@@tmp\@@tmp
    \expandafter\XC@add\@@tmp,\XC@@clr
  \fi}
\def\XC@split@v{\count@\z@ \expandafter\XC@split@vi\@@tmp!\@nil}
\def\XC@split@vi#1%
 {\ifx#1-\advance\count@\@ne\expandafter\XC@split@vi
  \else\expandafter\XC@split@vii\expandafter#1\fi}
\def\XC@split@vii#1!#2\@nil
 {\edef\@@nam{#1}\edef\@@mix{#2}%
  \ifodd\count@\@tempswatrue\else\@tempswafalse\fi
  \@ifundefined{\string\color@\@@nam}%
   {\c@lor@error{`\@@nam'}\def\@@nam{black}}{}%
  \let\xcolor@\@xcolor@\@nameuse{\string\color@\@@nam}}
\def\XC@postfix#1#2]#3\relax
 {\begingroup
  \if#1[\@tempcnta#2\relax\XC@stepabs\@@nam
  \else\@tempcnta\z@
    \@tfor\@@tok:=#1#2\do
     {\if\@@tok+\advance\@tempcnta\@ne
      \else\if\@@tok-\advance\@tempcnta\m@ne
      \else\@tempcnta\z@\expandafter\@break@tfor\fi\fi}%
    \ifnum\@tempcnta=\z@\relax\else\XC@step\@@nam\fi
    \let\@@tmp\@empty
  \fi\expandafter\endgroup\@@tmp}
\def\XC@display
 {\XC@bcolor\@namelet{\string\color@.}{XC@current@color}%
  \ifnum\XC@type{.}=1
    \PackageWarning{xcolor}{Incompatible color definition}%
  \else
    \ifnum\XC@tracing>2
      \begingroup \let\xcolor@\@empty \def\@nil{\string\@nil}%
      \PackageInfo{xcolor}{Setting color `\XC@current@color'}%
      \endgroup
    \fi
  \fi
  \XC@mcolor\set@color\XC@ecolor\ignorespaces}
\let\XC@bcolor\relax
\let\XC@mcolor\relax
\let\XC@ecolor\relax
\def\textcolor#1#{\@textcolor{#1}}
\def\@textcolor#1#2#3{\protect\leavevmode{\color#1{#2}#3}}
\def\color@block#1#2#3{%
 {\set@color\rlap{\ifcolors@\vrule\@width#1\@height#2\@depth#3\fi}}}
\def\colorbox#1#{\color@box{#1}}
\def\color@box#1#2{\color@b@x\relax{\color#1{#2}}}
\def\fcolorbox#1#{\color@fbox{#1}}
\def\color@fbox#1#2#3{%
  \color@b@x{\fboxsep\z@\color#1{#2}\fbox}{\color#1{#3}}}
\long\def\color@b@x#1#2#3{%
 \leavevmode
 \setbox\z@\hbox{\kern\fboxsep{\set@color#3}\kern\fboxsep}%
 \dimen@\ht\z@\advance\dimen@\fboxsep\ht\z@\dimen@
 \dimen@\dp\z@\advance\dimen@\fboxsep\dp\z@\dimen@
 {#1{#2\color@block{\wd\z@}{\ht\z@}{\dp\z@}%
      \box\z@}}}
\def\pagecolor
 {\begingroup
  \let\ignorespaces\endgroup \let\set@color\set@page@color
  \color}
\def\XC@bordercolor#1#2%
 {\extractcolorspec{#2}\XC@@tmp
  \expandafter\convertcolorspec\XC@@tmp\XC@mod@rgb\XC@@tmp
  \expandafter\edef\csname @#1bordercolor\endcsname
   {\expandafter\XC@@bordercolor\XC@@tmp,}}
\def\XC@@bordercolor#1,#2,#3,{#1 #2 #3}
\def\XC@pdfborder#1 #2 #3\relax
 {\def\@@scl{80}\XC@calc@#1,#2,#3,,:S%
  \edef\@pdfborder{\expandafter\XC@@bordercolor\@@tmp,}}
\AtBeginDocument{\@ifundefined{ver@colortbl.sty}{}{%
 \def\rowcolors{\@ifstar{\@rowcmdfalse\rowc@lors}{\@rowcmdtrue\rowc@lors}}%
 \def\rowc@lors{\@testopt{\rowc@l@rs}{}}%
 \def\rowc@l@rs[#1]#2#3#4%
  {\global\rownum=\z@
   \global\@rowcolorstrue
   \@ifxempty{#3}%
     {\def\@oddrowcolor{\@norowcolor}}%
     {\def\@oddrowcolor{\gdef\CT@row@color{\CT@color{#3}}}}%
   \@ifxempty{#4}%
     {\def\@evenrowcolor{\@norowcolor}}%
     {\def\@evenrowcolor{\gdef\CT@row@color{\CT@color{#4}}}}%
   \if@rowcmd
     \def\@rowcolors
      {#1\if@rowcolors
         \noalign{\relax\ifnum\rownum<#2\@norowcolor\else
                  \ifodd\rownum\@oddrowcolor\else\@evenrowcolor\fi\fi}%
       \fi}%
   \else
     \def\@rowcolors
      {\if@rowcolors
         \ifnum\rownum<#2\noalign{\@norowcolor}\else
         #1\noalign{\ifodd\rownum\@oddrowcolor\else\@evenrowcolor\fi}\fi
       \fi}%
   \fi
   \CT@everycr{\noalign{\rownum@step}\@rowcolors\the\everycr}%
   \ignorespaces}%
 \def\showrowcolors{\noalign{\global\@rowcolorstrue}\@rowcolors}%
 \def\hiderowcolors{\noalign{\global\@rowcolorsfalse\@norowcolor}}%
 \def\@norowcolor{\global\let\CT@row@color\relax}%
 \newif\if@rowcolors
 \newif\if@rowcmd
 \ifx\rownum\@undefined\newcount\rownum\fi
 \def\rownum@step{\global\advance\rownum\@ne}%
 \def\CT@extract#1\columncolor#2#3\@nil{%
   \if!#2%
     \let\CT@column@color\@empty
   \else
     \if[#2%
       \CT@extractb{#1}#3\@nil
     \else
       \XC@edef\XC@@tmp{#2}%
       \edef\CT@column@color{\noexpand\CT@color{\XC@@tmp}}%
       \CT@extractd{#1}#3\@nil
     \fi
   \fi}%
 }}
\def\extractcolorspec#1#2%
 {\XC@split{#1}\aftergroupdef#2{{\@@mod}{\@@clr}}}
\def\XC@extract@hue#1,#2:#3{\edef#3{#1}}
\def\XC@type#1%
 {\expandafter\expandafter\expandafter\XC@@type
  \csname\string\color@#1\endcsname\@empty\@empty\@empty\XC@@}
\def\XC@@type#1#2#3#4\XC@@
 {\ifx#1\relax 0\else
    \ifx#1\xcolor@
      \ifx$#2$%
        \ifx$#3$4\else3\fi\@gobbletwo
      \else2\fi\@gobbletwo
    \else1\fi
  \fi}
\def\tracingcolors{\begingroup\afterassignment\XC@tracingcolors\count@}
\def\XC@tracingcolors{\aftergroupdef\XC@tracing{\the\count@}}
\tracingcolors=0
\def\XC@logdef#1%
 {\ifnum\XC@tracing>1
    \@ifundefined{\string\color@#1}%
     {\ifnum\XC@tracing>2
        \PackageInfo{xcolor}{Defining color `#1'}%
      \fi}%
     {\PackageInfo{xcolor}{Redefining color `#1'}}%
  \fi}
\def\color@setgroup{\begingroup\set@color}
\let\color@begingroup\begingroup
\def\color@endgroup{\endgraf\endgroup}
\def\color@hbox{\hbox\bgroup\color@begingroup}
\def\color@vbox{\vbox\bgroup\color@begingroup}
\def\color@endbox{\color@endgroup\egroup}
\def\convertcolorspec#1#2#3#4%
 {\begingroup
  \edef\sm{#1}\edef\tm{#3}\edef\@@tmp{#2}%
  \ifx\sm\XC@mod@named
    \extractcolorspec\@@tmp\@@tmp
    \edef\sm{\expandafter\@firstoftwo\@@tmp}%
    \edef\@@tmp{\expandafter\@secondoftwo\@@tmp}%
  \fi
  \ifx\sm\tm\else\csname XC@cnv@\sm\expandafter\endcsname\@@tmp,\fi
  \aftergroupdef#4\@@tmp}
\def\XC@coremodel#1#2%
 {\ifx#1\XC@mod@RGB
    \convertcolorspec#1#2\XC@mod@rgb#2\let#1\XC@mod@rgb\else
  \ifx#1\XC@mod@HTML
    \convertcolorspec#1#2\XC@mod@rgb#2\let#1\XC@mod@rgb\else
  \ifx#1\XC@mod@HSB
    \convertcolorspec#1#2\XC@mod@hsb#2\let#1\XC@mod@hsb\else
  \ifx#1\XC@mod@Gray
    \convertcolorspec#1#2\XC@mod@gray#2\let#1\XC@mod@gray\else
  \ifx#1\XC@mod@named\else
  \expandafter\XC@calc@#2,,,,:N\let#2\@@tmp
  \fi\fi\fi\fi\fi}
\def\XC@cnv@rgb#1,#2,#3,%
 {\ifx\tm\XC@mod@cmy
    \XC@calc@#1,#2,#3,,:C%
  \else\ifx\tm\XC@mod@cmyk
    \XC@calc@#1,#2,#3,,:C\expandafter\XC@cnv@cmy@cmyk\@@tmp,%
  \else\ifx\tm\XC@mod@hsb
    \XC@cnv@rgb@hsb#1,#2,#3,%
  \else\ifx\tm\XC@mod@gray
    \XC@cnv@rgb@gray#1,#2,#3,%
  \else\ifx\tm\XC@mod@RGB
    \edef\@@scl{\rangeRGB}\XC@calc@#1,#2,#3,,:M%
  \else\ifx\tm\XC@mod@HTML
    \edef\@@scl{\@cclv}\XC@calc@#1,#2,#3,,:M%
    \expandafter\XC@calc@\@@tmp,,:H%
    \expandafter\XC@cnv@rgb@HTML\@@tmp,%
  \else\ifx\tm\XC@mod@HSB
    \XC@cnv@rgb@hsb#1,#2,#3,%
    \edef\@@scl{\rangeHSB}\expandafter\XC@calc@\@@tmp,,:M%
  \else\ifx\tm\XC@mod@Gray
    \XC@cnv@rgb@gray#1,#2,#3,%
    \edef\@@scl{\rangeGray}\XC@calcM\@@tmp\@@tmp
  \else
    \XC@calc@#1,#2,#3,,:N%
  \fi\fi\fi\fi\fi\fi\fi\fi}
\def\XC@cnv@rgb@hsb#1,#2,#3,%
 {\count@\z@
  \ifdim#2\p@>#1\p@ \else\advance\count@4 \fi
  \ifdim#3\p@>#2\p@ \else\advance\count@2 \fi
  \ifdim#1\p@>#3\p@ \else\advance\count@1 \fi
  \ifcase\count@\or
  \XC@@cnv@rgb@hsb{#3}{#2}{#1}3{}\or
  \XC@@cnv@rgb@hsb{#2}{#1}{#3}1{}\or
  \XC@@cnv@rgb@hsb{#2}{#3}{#1}3-\or
  \XC@@cnv@rgb@hsb{#1}{#3}{#2}5{}\or
  \XC@@cnv@rgb@hsb{#3}{#1}{#2}5-\or
  \XC@@cnv@rgb@hsb{#1}{#2}{#3}1-\or
  \def\@tempa{0}\def\@tempb{0}\XC@calcN{#3}\@tempc
  \fi
  \edef\@@tmp{\@tempa,\@tempb,\@tempc}}
\def\XC@@cnv@rgb@hsb#1#2#3#4#5%
 {\XC@calcN{#1}\@tempc \llshiftset\dimen@{#1}%
  \llshiftset\@tempdimb{-#3}\advance\@tempdimb\dimen@
  \llshiftset\@tempdima{-#5#2}\advance\@tempdima#5\dimen@
  \advance\@tempdima#4\@tempdimb \rdivide\@tempdima{6\@tempdimb}%
  \edef\@tempa{\ifdim\@tempdima>\p@1\else\strip@pt\@tempdima\fi}%
  \rdivide\@tempdimb\dimen@
  \edef\@tempb{\strip@pt\@tempdimb}}
\def\XC@cnv@rgb@gray#1,#2,#3,%
 {\llshiftset\dimen@{#1}\@tempdima30\dimen@
  \llshiftset\dimen@{#2}\advance\@tempdima59\dimen@
  \llshiftset\dimen@{#3}\advance\@tempdima11\dimen@
  \rrshift\@tempdima \rdivide\@tempdima{100}%
  \edef\@@tmp{\strip@pt\@tempdima}}
\def\XC@cnv@rgb@HTML#1,#2,#3,%
 {\edef\@@tmp{#1#2#3}}
\def\XC@cnv@cmy#1,#2,#3,%
 {\ifx\tm\XC@mod@rgb
    \XC@calc@#1,#2,#3,,:C%
  \else\ifx\tm\XC@mod@cmyk
    \XC@cnv@cmy@cmyk#1,#2,#3,%
  \else\ifx\tm\XC@mod@hsb
    \XC@calc@#1,#2,#3,,:C\expandafter\XC@cnv@rgb@hsb\@@tmp,%
  \else\ifx\tm\XC@mod@gray
    \XC@cnv@rgb@gray#1,#2,#3,\XC@calcC\@@tmp\@@tmp
  \else\ifx\tm\XC@mod@RGB
    \XC@calc@#1,#2,#3,,:C%
    \edef\@@scl{\rangeRGB}\expandafter\XC@calc@\@@tmp,,:M%
  \else\ifx\tm\XC@mod@HTML
    \XC@calc@#1,#2,#3,,:C\expandafter\XC@cnv@rgb\@@tmp,%
  \else\ifx\tm\XC@mod@HSB
    \XC@calc@#1,#2,#3,,:C\expandafter\XC@cnv@rgb@hsb\@@tmp,%
    \edef\@@scl{\rangeHSB}\expandafter\XC@calc@\@@tmp,,:M%
  \else\ifx\tm\XC@mod@Gray
    \XC@cnv@rgb@gray#1,#2,#3,\XC@calcC\@@tmp\@@tmp
    \edef\@@scl{\rangeGray}\XC@calcM\@@tmp\@@tmp
  \else
    \XC@calc@#1,#2,#3,,:N%
  \fi\fi\fi\fi\fi\fi\fi\fi}
\def\XC@cnv@cmy@cmyk#1,#2,#3,%
 {\edef\@@scl
   {\ifdim#1\p@<#2\p@
    \ifdim#1\p@<#3\p@ #1\else #3\fi \else
    \ifdim#2\p@<#3\p@ #2\else #3\fi \fi}%
  \expandafter\XC@calc@\adjustUCRBG,:S%
  \expandafter\XC@@cnv@cmy@cmyk\@@tmp,#1,#2,#3,}
\def\XC@@cnv@cmy@cmyk#1,#2,#3,#4,#5,#6,#7,%
 {\XC@add#5,#6,#7,,-#1,-#2,-#3,,\@@tmp \edef\@@tmp{\@@tmp,#4}%
  \expandafter\XC@calc@\@@tmp,:N}
\def\XC@cnv@cmyk#1,#2,#3,#4,%
 {\ifx\tm\XC@mod@rgb
    \XC@cnv@cmyk@cmy#1,#2,#3,#4,\expandafter\XC@calc@\@@tmp,,:C%
  \else\ifx\tm\XC@mod@cmy
    \XC@cnv@cmyk@cmy#1,#2,#3,#4,%
  \else\ifx\tm\XC@mod@hsb
    \XC@cnv@cmyk@cmy#1,#2,#3,#4,\expandafter\XC@calc@\@@tmp,,:C%
    \expandafter\XC@cnv@rgb@hsb\@@tmp,%
  \else\ifx\tm\XC@mod@gray
    \XC@cnv@rgb@gray#1,#2,#3,%
    \edef\@@arg{#4}\XC@calcT\@@tmp\@@tmp \XC@calcC\@@tmp\@@tmp
  \else\ifx\tm\XC@mod@RGB
    \XC@cnv@cmyk@cmy#1,#2,#3,#4,\expandafter\XC@calc@\@@tmp,,:C%
    \edef\@@scl{\rangeRGB}\expandafter\XC@calc@\@@tmp,,:M%
  \else\ifx\tm\XC@mod@HTML
    \XC@cnv@cmyk@cmy#1,#2,#3,#4,\expandafter\XC@cnv@cmy\@@tmp,%
  \else\ifx\tm\XC@mod@HSB
    \XC@cnv@cmyk@cmy#1,#2,#3,#4,\expandafter\XC@calc@\@@tmp,,:C%
    \expandafter\XC@cnv@rgb@hsb\@@tmp,%
    \edef\@@scl{\rangeHSB}\expandafter\XC@calc@\@@tmp,,:M%
  \else\ifx\tm\XC@mod@Gray
    \XC@cnv@rgb@gray#1,#2,#3,%
    \edef\@@arg{#4}\XC@calcT\@@tmp\@@tmp \XC@calcC\@@tmp\@@tmp
    \edef\@@scl{\rangeGray}\XC@calcM\@@tmp\@@tmp
  \else
    \XC@calc@#1,#2,#3,#4,:N%
  \fi\fi\fi\fi\fi\fi\fi\fi}
\def\XC@cnv@cmyk@cmy#1,#2,#3,#4,%
 {\edef\@@arg{#4}\XC@calc@#1,#2,#3,,:T}
\def\XC@cnv@hsb#1,#2,#3,%
 {\ifx\tm\XC@mod@HSB
    \edef\@@scl{\rangeHSB}\XC@calc@#1,#2,#3,,:M%
  \else
    \XC@cnv@hsb@rgb#1,#2,#3,%
    \ifx\tm\XC@mod@rgb\else\expandafter\XC@cnv@rgb\@@tmp,\fi
  \fi}
\def\XC@cnv@hsb@rgb#1,#2,#3,%
 {\llshiftset\dimen@{#1}\dimen@6\dimen@ \rrshift\dimen@
  \afterassignment\dimen@\count@=\the\dimen@
  \edef\@@tmp{\strip@pt\dimen@}%
  \ifodd\count@\else\XC@calcC\@@tmp\@@tmp\fi
  \edef\@@tmp
   {\ifcase\count@ 0,\@@tmp,1\or \@@tmp,0,1\or 1,0,\@@tmp\or
    1,\@@tmp,0\or \@@tmp,1,0\or 0,1,\@@tmp\or 0,\@@tmp,1\fi}%
  \edef\@@scl{#2}\expandafter\XC@calc@\@@tmp,,:S%
  \expandafter\XC@calc@\@@tmp,,:C%
  \edef\@@scl{#3}\expandafter\XC@calc@\@@tmp,,:S}
\def\XC@cnv@gray#1,%
 {\ifx\tm\XC@mod@rgb
    \XC@calcN{#1}\@@tmp \edef\@@tmp{\@@tmp,\@@tmp,\@@tmp}%
  \else\ifx\tm\XC@mod@cmy
    \XC@calcC{#1}\@@tmp \edef\@@tmp{\@@tmp,\@@tmp,\@@tmp}%
  \else\ifx\tm\XC@mod@cmyk
    \XC@calcC{#1}\@@tmp \edef\@@tmp{0,0,0,\@@tmp}%
  \else\ifx\tm\XC@mod@hsb
    \XC@calcN{#1}\@@tmp \edef\@@tmp{0,0,\@@tmp}%
  \else\ifx\tm\XC@mod@RGB
    \edef\@@scl{\rangeRGB}\XC@calcM{#1}\@@tmp
    \edef\@@tmp{\@@tmp,\@@tmp,\@@tmp}%
  \else\ifx\tm\XC@mod@HTML
    \edef\@@scl{\@cclv}\XC@calcM{#1}\@@tmp \XC@calcH\@@tmp\@@tmp
    \edef\@@tmp{\@@tmp\@@tmp\@@tmp}%
  \else\ifx\tm\XC@mod@HSB
    \edef\@@scl{\rangeHSB}\XC@calcM{#1}\@@tmp
    \edef\@@tmp{0,0,\@@tmp}%
  \else\ifx\tm\XC@mod@Gray
    \edef\@@scl{\rangeGray}\XC@calcM{#1}\@@tmp
  \else
    \XC@calcN{#1}\@@tmp
  \fi\fi\fi\fi\fi\fi\fi\fi}
\def\XC@cnv@RGB#1,#2,#3,%
 {\edef\@@scl{\rangeRGB}\XC@calc@#1,#2,#3,,:D\expandafter\XC@cnv@rgb\@@tmp,}
\def\XC@cnv@HTML#1,%
 {\edef\@@tmp{\expandafter\@hex@Hex#1\relax}\expandafter\XC@cnv@HTML@\@@tmp
  \edef\@@scl{\@cclv}\expandafter\XC@calc@\@@tmp,,:D%
  \expandafter\XC@cnv@rgb\@@tmp,}
\def\XC@cnv@HTML@#1#2#3#4#5#6%
 {\edef\@@tmp{\number"#1#2,\number"#3#4,\number"#5#6}}
\def\XC@cnv@HSB#1,#2,#3,%
 {\edef\@@scl{\rangeHSB}\XC@calc@#1,#2,#3,,:D\expandafter\XC@cnv@hsb\@@tmp,}
\def\XC@cnv@Gray#1,%
 {\edef\@@scl{\rangeGray}\XC@calcD{#1}\@@tmp \XC@cnv@gray\@@tmp,}
\def\XC@cnv@cmyk@compl#1,#2,#3,#4,%
 {\XC@cnv@cmyk@cmy#1,#2,#3,#4,%
  \expandafter\XC@calc@\@@tmp,,:C%
  \expandafter\XC@cnv@cmy@cmyk\@@tmp,}
\def\XC@cnv@hsb@compl#1,#2,#3,%
 {\lshiftset\dimen@{#1}\advance\dimen@\ifdim\dimen@<5\p@-\fi-5\p@
  \rshift\dimen@
  \edef\@@tmp{\strip@pt\dimen@}%
  \lshiftset\dimen@{#3}%
  \@tempdima#2\dimen@
  \@tempdimb\@tempdima \advance\@tempdimb10\p@ \advance\@tempdimb-\dimen@
  \ifdim\@tempdimb=\z@
    \edef\@@tmp{\@@tmp,0,0}%
  \else
    \rdivide\@tempdima\@tempdimb \rshift\@tempdimb
    \edef\@@tmp{\@@tmp,\strip@pt\@tempdima,\strip@pt\@tempdimb}%
  \fi}
\ifx\color@rgb\@undefined
  \PackageInfo{xcolor}{Color model `rgb' added}
  \def\color@rgb#1#2%
   {\convertcolorspec\XC@mod@rgb{#2}\XC@mod@cmyk\XC@@tmp
    \expandafter\color@cmyk\expandafter#1\expandafter{\XC@@tmp}}
\fi
\ifx\color@cmyk\@undefined
  \PackageInfo{xcolor}{Color model `cmyk' added}
  \def\color@cmyk#1#2%
   {\convertcolorspec\XC@mod@cmyk{#2}\XC@mod@rgb\XC@@tmp
    \expandafter\color@rgb\expandafter#1\expandafter{\XC@@tmp}}
\fi
\ifx\color@cmy\@undefined
  \PackageInfo{xcolor}{Color model `cmy' added}
  \def\color@cmy#1#2{\color@cmyk#1{#2,0}}
\fi
\ifx\color@hsb\@undefined\@tempswatrue
\else\def\@@tmp{dvipdfm.def}\ifx\@@tmp\Gin@driver\@tempswatrue
\else\def\@@tmp{textures.def}\ifx\@@tmp\Gin@driver\@tempswatrue
\else\@tempswafalse\fi\fi\fi
\if@tempswa
  \PackageInfo{xcolor}{Color model `hsb' added}
  \def\color@hsb#1#2%
   {\convertcolorspec\XC@mod@hsb{#2}\XC@mod@rgb\XC@@tmp
    \expandafter\color@rgb\expandafter#1\expandafter{\XC@@tmp}}
\fi
\ifx\color@gray\@undefined
  \PackageInfo{xcolor}{Color model `gray' added}
  \def\color@gray#1#2{\color@rgb#1{#2,#2,#2}}
\fi
\ifx\color@RGB\@undefined\@tempswatrue
\else\ifnum\rangeRGB<255 \@tempswatrue
\else\ifnum\rangeRGB>255 \@tempswatrue
\else\@tempswafalse\fi\fi\fi
\if@tempswa
  \PackageInfo{xcolor}{Color model `RGB' added}
  \def\color@RGB#1#2%
   {\convertcolorspec\XC@mod@RGB{#2}\XC@mod@rgb\XC@@tmp
    \expandafter\color@rgb\expandafter#1\expandafter{\XC@@tmp}}
\fi
\ifx\color@HTML\@undefined
  \PackageInfo{xcolor}{Color model `HTML' added}
  \def\color@HTML#1#2%
   {\convertcolorspec\XC@mod@HTML{#2}\XC@mod@rgb\XC@@tmp
    \expandafter\color@rgb\expandafter#1\expandafter{\XC@@tmp}}
\fi
\ifx\color@HSB\@undefined
  \PackageInfo{xcolor}{Color model `HSB' added}
  \def\color@HSB#1#2%
   {\convertcolorspec\XC@mod@HSB{#2}\XC@mod@hsb\XC@@tmp
    \expandafter\color@hsb\expandafter#1\expandafter{\XC@@tmp}}
\fi
\ifx\color@Gray\@undefined
  \PackageInfo{xcolor}{Color model `Gray' added}
  \def\color@Gray#1#2%
   {\convertcolorspec\XC@mod@Gray{#2}\XC@mod@gray\XC@@tmp
    \expandafter\color@gray\expandafter#1\expandafter{\XC@@tmp}}
\fi
\@ifundefined{XC@pst}{%
\def\XC@getcolor#1#2%
 {\begingroup
  \XC@@getcolor#1\XC@@
  \toks@\expandafter{\@@tmp}\aftergroupdef#2{\the\toks@}}
\def\XC@@getcolor#1#2\XC@@
 {\@ifxempty{#2}%
   {\expandafter\XC@@@getcolor#1\XC@@}%
   {\color{#1#2}\let\@@tmp\XC@current@color}}
\def\XC@@@getcolor#1#2\XC@@
 {\ifx#1\xcolor@
    \def\@@tmp{\xcolor@#2}%
  \else
    \color{#1#2}\let\@@tmp\XC@current@color
  \fi}
}{% compatibility code begin
\def\XC@getcolor#1#2%
 {\@ifundefined{\string\color@#1}%
   {\begingroup\color{#1}%
    \edef\@@tmp
     {\noexpand\edef\noexpand#2{\noexpand\expandafter\noexpand\c@lor@to@ps
      \current@color\noexpand\@@}}%
    \expandafter\endgroup\@@tmp}%
   {\edef#2{\XC@usecolor{#1}}}}
}% compatibility code end
\def\XC@usecolor#1{\expandafter\XC@@usecolor#1\XC@@}
\def\XC@@usecolor#1#2\XC@@
 {\ifx#1\xcolor@
    \expandafter\expandafter\expandafter\c@lor@to@ps#1#2\@@
  \else
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
    \expandafter\c@lor@to@ps\csname\string\color@#1#2\endcsname\@@
  \fi
  \space}
\let\XC@c@lor@to@ps\XC@usecolor
\let\pst@getcolor\XC@getcolor
\@ifundefined{XC@pst}{%
  \let\pst@usecolor\XC@usecolor
}{}
\def\c@lor@special#1#2{\edef\@tempa{\write#1{#2}}\@tempa}
\def\normalcolor{\let\current@color\default@color\set@color}
\AtBeginDocument{\let\default@color\current@color}
\@tfor\@@tmp:={dvipdf}{dvipdfm}{dvips}{pctex32}\do
 {\edef\@@tmp{\@@tmp.def}%
  \ifx\Gin@driver\@@tmp
    \def\c@lor@@named#1,#2,#3\@@#4{\edef#4{ #1}}
    \def\define@color@named#1#2{\let\@@col\@nnil}
  \@break@tfor\fi}
\@tfor\@@tmp:={dvipsone}{pctexps}{pdftex}{tcidvi}{truetex}{vtex}\do
 {\edef\@@tmp{\@@tmp.def}%
  \ifx\Gin@driver\@@tmp
    \def\c@lor@@named#1,#2,#3\@@#4%
     {\edef#4{\expandafter\expandafter\expandafter\@secondoffive
               \csname\string\color@#1\endcsname}}
    \def\define@color@named#1#2%
     {\edef\@@col{#2}\@namedef{\string\color@#1}{{}{#2}{}{}{}}}
  \@break@tfor\fi}
\@tfor\@@tmp:={textures}\do
 {\edef\@@tmp{\@@tmp.def}%
  \ifx\Gin@driver\@@tmp
    \def\c@lor@@named#1,#2,#3\@@#4%
     {\edef\@tempa{\color@P@custom{#1}{\if!#2!1\else#2\fi}}%
      \expandafter\def\expandafter#4\@tempa}
    \def\define@color@named#1#2%
     {\edef\@tempa{{#1}{#2}}\expandafter\AddCustomColor\@tempa
      \edef\@@col{#2}}
  \@break@tfor\fi}
\definecolorset{rgb}{}{}{red,1,0,0;green,0,1,0;blue,0,0,1}
\definecolorset{cmyk}{}{}{cyan,1,0,0,0;magenta,0,1,0,0;yellow,0,0,1,0}
\definecolorset{gray}{}{}{black,0;darkgray,.25;gray,.5;lightgray,.75;white,1}
\colorlet{orange}{red!50!yellow}
\colorlet{violet}{blue!50!red}
\colorlet{purple}{violet!50!red}
\colorlet{brown}{violet!50!yellow}
\XC@colornames
\XC@catcodes
\let\XC@catcodes\relax
\@nameuse{xcolorcmd}
\color{black}
\endinput
%%
%% End of file `xcolor.sty'.

